AnyDB: An Architecture-less DBMS for Any Workload

In this paper, we propose a radical new approach for scale-out distributed DBMSs. Instead of hard-baking an architectural model, such as a shared-nothing architecture, into the distributed DBMS design, we aim for a new class of so-called architecture-less DBMSs. The main idea is that an architecture-less DBMS can mimic any architecture on a per-query basis on-the-fly without any additional overhead for reconfiguration. Our initial results show that our architecture-less DBMS AnyDB can provide significant speed-ups across varying workloads compared to a traditional DBMS implementing a static architecture.

==> figures/plots/Main-Experiment_OLAP/Main-Experiment_OLAP-throughput_query_per_second.tex <==
% This file was created by tikzplotlib v0.9.0.
\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}

\begin{axis}[
axis line style={white!15!black},
height=\figH,
tick pos=left,
title style={yshift=-1.5ex},
title={OLAP Performance},
width=\figW,
x grid style={white!80!black},
xlabel shift=-1ex,
xlabel={Workload Phase},
xmajorticks=true,
xmin=8.375, xmax=11.125,
xtick style={color=white!15!black},
xtick={8,8.5,9,9.5,10,10.5,11,11.5},
xticklabel style={align=left},
xticklabels={8.75,9.00,9.25,9.50,9.75,10.00,10.25,10.50},
y grid style={white!80!black},
ylabel shift=-1.4ex,
ylabel={throughput\_query\_per\_second},
ymin=0, ymax=18.3727459875,
yminorticks=false,
ytick style={color=white!15!black},
ytick={0,2.5,5,7.5,10,12.5,15,17.5,20},
yticklabels={0,2,4,6,8,10,12,14,16}
]
\path [draw=color0, line width=0.48pt]
(axis cs:9,2.19327)
--(axis cs:9,2.19627);

\path [draw=color0, line width=0.48pt]
(axis cs:10,2.19087)
--(axis cs:10,2.19641);

\path [draw=color0, line width=0.48pt]
(axis cs:11,2.19544)
--(axis cs:11,2.19925);

\path [draw=color0, line width=0.48pt]
(axis cs:9,9.72381)
--(axis cs:9,9.79545);

\path [draw=color0, line width=0.48pt]
(axis cs:10,9.72602)
--(axis cs:10,9.79619);

\path [draw=color0, line width=0.48pt]
(axis cs:11,9.75546)
--(axis cs:11,9.83078);

\path [draw=color0, line width=0.48pt]
(axis cs:9,16.2774)
--(axis cs:9,16.3485);

\path [draw=color0, line width=0.48pt]
(axis cs:10,16.29)
--(axis cs:10,16.3775);

\path [draw=color0, line width=0.48pt]
(axis cs:11,16.2116)
--(axis cs:11,16.3814);

\path [draw=color1, line width=0.48pt]
(axis cs:9,6.52237)
--(axis cs:9,6.54169);

\path [draw=color1, line width=0.48pt]
(axis cs:10,6.51174)
--(axis cs:10,6.52165);

\path [draw=color1, line width=0.48pt]
(axis cs:11,6.50206)
--(axis cs:11,6.53891);

\addplot [line width=0.48pt, color0, mark=*, mark size=2, mark options={solid,draw=white}]
table {%
9 2.19475
10 2.19341
11 2.19815
};
\addplot [line width=0.48pt, color0, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}]
table {%
9 9.76153
10 9.76791
11 9.79376
};
\addplot [line width=0.48pt, color0, dash pattern=on 1pt off 1pt, mark=pentagon*, mark size=2, mark options={solid,draw=white}]
table {%
9 16.3225
10 16.295
11 16.3423
};
\addplot [line width=0.48pt, color1, dash pattern=on 1pt off 1pt, mark=pentagon*, mark size=2, mark options={solid,draw=white}]
table {%
9 6.53473
10 6.52017
11 6.51508
};
\addplot [line width=0.48pt, white!50.1960784313725!black, dashed]
table {%
8.5 0
8.5 18.3727459875
};
\addplot [line width=0.48pt, color0]
table {%
9 2.19475
10 2.19341
11 2.19815
};
\addplot [line width=0.48pt, color0]
table {%
9 9.76153
10 9.76791
11 9.79376
};
\addplot [line width=0.48pt, color0]
table {%
9 16.3225
10 16.295
11 16.3423
};
\addplot [line width=0.48pt, color1]
table {%
9 6.53473
10 6.52017
11 6.51508
};
\draw (axis cs:10,16.9029263085) node[
  scale=0.6,
  anchor=base,
  text=white!15!black,
  rotate=0.0,
  align=center
]{HTAP
partitionable};
\end{axis}



==> figures/plots/Microbench_Data-Beam/Microbench_Data-Beam-duration_ns.tex <==
% This file was created by tikzplotlib v0.9.0.
\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color3}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}

\begin{axis}[
legend entries={baseline, beam build, beam both, pipelined, Compile time DB-Y},
axis line style={white!15!black},
height=\figH,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1,1)}, anchor=north west, draw=white!80!black},
tick pos=left,
title style={yshift=-1.5ex},
width=\figW,
x grid style={white!80!black},
xlabel shift=-1ex,
xlabel={Query Compile Time (us)},
xmajorticks=true,
xmin=-950, xmax=41950,
xtick style={color=white!15!black},
xticklabel style={align=left},
y grid style={white!80!black},
ylabel shift=-1.4ex,
ylabel={duration\_ns},
ymin=0, ymax=64831746.65,
yminorticks=false,
ytick style={color=white!15!black},
%ytick={0,10000000,20000000,30000000,40000000,50000000,60000000,70000000},
%yticklabels={0,1,2,3,4,5,6,7}
]
\addplot [line width=0.48pt, color0, mark=*, mark size=2, mark options={solid,draw=white}]
table {%
1000 25673724
5000 27250270
10000 32195845
20000 42107525
30000 51908189
40000 62318697
};
\addplot [line width=0.48pt, color0, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 21553230
5000 25481229
10000 30527279
20000 40605994
30000 50451505
40000 60451320
};
\addplot [line width=0.48pt, color1, mark=*, mark size=2, mark options={solid,draw=white}]
table {%
1000 18409612
5000 18491472
10000 23037559
20000 32980654
30000 42817835
40000 52829454
};
\addplot [line width=0.48pt, color1, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 17292121
5000 17281872
10000 21786974
20000 31835135
30000 41885774
40000 51851182
};
\addplot [line width=0.48pt, color2, mark=*, mark size=2, mark options={solid,draw=white}]
table {%
1000 12618120
5000 12419266
10000 14510197
20000 24458719
30000 34525089
40000 44519748
};
\addplot [line width=0.48pt, color2, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 12120013
5000 12176784
10000 12866216
20000 22816423
30000 32813461
40000 42768902
};
\addplot [line width=0.48pt, color3, mark=*, mark size=2, mark options={solid,draw=white}]
table {%
1000 12057704
5000 12291627
10000 12568286
20000 12306512
30000 12894983
40000 12400501
};
\addplot [line width=0.48pt, color3, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 12260388
5000 12293857
10000 12136385
20000 12186101
30000 12108130
40000 12123751
};
\addplot [line width=0.48pt, black, dashed]
table {%
30000 9.31322574615479e-10
30000 64831746.65
};
\end{axis}



==> figures/plots/Microbench_Data-Beam/Microbench_Data-Beam-probe_time.tex <==
% This file was created by tikzplotlib v0.9.0.
\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color3}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}

\begin{axis}[
axis line style={white!15!black},
height=\figH,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.03)}, anchor=south west, draw=white!80!black},
tick pos=left,
title style={yshift=-1.5ex},
width=\figW,
x grid style={white!80!black},
xlabel shift=-1ex,
xlabel={Query Compile Time (us)},
xmajorticks=true,
xmin=-950, xmax=41950,
xtick style={color=white!15!black},
xticklabel style={align=left},
y grid style={white!80!black},
ylabel shift=-1.4ex,
ylabel={probe\_time},
ymin=0, ymax=29900101.5,
yminorticks=false,
ytick style={color=white!15!black},
ytick={0,5000000,10000000,15000000,20000000,25000000,30000000},
yticklabels={0.0,0.5,1.0,1.5,2.0,2.5,3.0}
]
\addplot [line width=0.48pt, color0, mark=*, mark size=2, mark options={solid,draw=white}, forget plot]
table {%
1000 28548872
5000 28514399
10000 28454437
20000 28678854
30000 28115347
40000 28569063
};
\addplot [line width=0.48pt, color0, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 27477803
5000 27506901
10000 27496466
20000 27640451
30000 27418618
40000 27444133
};
\addplot [line width=0.48pt, color1, mark=*, mark size=2, mark options={solid,draw=white}, forget plot]
table {%
1000 24903688
5000 24130514
10000 23471072
20000 22948017
30000 23025347
40000 23061116
};
\addplot [line width=0.48pt, color1, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 24141983
5000 22791899
10000 22232179
20000 22182136
30000 22288048
40000 22311159
};
\addplot [line width=0.48pt, color2, mark=*, mark size=2, mark options={solid,draw=white}, forget plot]
table {%
1000 11331728
5000 11671104
10000 6606977
20000 6482157
30000 6623787
40000 6567557
};
\addplot [line width=0.48pt, color2, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 13528264
5000 12473267
10000 4356693
20000 4261833
30000 4328463
40000 4253904
};
\addplot [line width=0.48pt, color3, mark=*, mark size=2, mark options={solid,draw=white}, forget plot]
table {%
1000 11838599
5000 11773692
10000 13084880
20000 12338497
30000 13119125
40000 12379509
};
\addplot [line width=0.48pt, color3, dash pattern=on 4pt off 1.5pt, mark=triangle*, mark size=2, mark options={solid,rotate=180,draw=white}, forget plot]
table {%
1000 13623851
5000 13798330
10000 13658395
20000 13637659
30000 13462402
40000 13556854
};
\addplot [line width=0.48pt, black, dashed, forget plot]
table {%
30000 4.65661287307739e-10
30000 29900101.5
};
\end{axis}


